Manu: A Cloud Native Vector Database Management System

With the development of learning-based embedding models, embedding vectors are widely used for analyzing and searching unstructured data. As vector collections exceed billion-scale, fully managed and horizontally scalable vector databases are necessary. In the past three years, through interaction with our 1200+ industry users, we have sketched a vision for the features that next-generation vector databases should have, which include long-term evolvability, tunable consistency, good elasticity, and high performance. We present Manu, a cloud native vector database that implements these features. It is difficult to integrate all these features if we follow traditional DBMS design rules. As most vector data applications do not require complex data models and strong data consistency, our design philosophy is to relax the data model and consistency constraints in exchange for the aforementioned features. Specifically, Manu firstly exposes the write-ahead log (WAL) and binlog as backbone services. Secondly, write components are designed as log publishers while all read-only analytic and search components are designed as independent subscribers to the log services. Finally, we utilize multi-version concurrency control (MVCC) and a delta consistency model to simplify the communication and cooperation among the system components. These designs achieve a low coupling among the system components, which is essential for elasticity and evolution. We also extensively optimize Manu for performance and usability with hardware-aware implementations and support for complex search semantics.

==> figures/7_rela.tex <==
\section{Related work}\label{sec:rel}

In this part, we review works that are most relevant to ours.

\stitle{Traditional cardinality estimators} \emph{Histogram-based} cardinality estimation methods~\cite{deshpande2001independence, aboulnaga1999self, gunopulos2005selectivity} have been widely used in many industrial database systems as they are simple and have very low overhead.
However, they lack the ability to capture the data correlations among the tables as they make the attribute-value-independence assumption.
\emph{Sampling-based} approaches~\cite{chen2017two, ganguly1996bifocal, vengerov2015join} outperform histogram-based methods as the correlations in data are naturally captured by data samples.
However, sampling-based approaches have two limitations: (i) empty sampling set of join result; and (ii) high sampling overhead.
Recent works~\cite{yu2013cs2, leis2017cardinality} have proposed index-based and materialized sampling strategies to alleviate the problem of empty result. However, it is still difficult to use sampling to evaluate the cost of all execution plans as it incurs high space- and time- costs.



\stitle{Learning-based cardinality estimators}
%With the advance of machine and deep learning techniques, researchers proposed many learning-based solutions for various problems~\cite{kraska2018case,krishnan2018learning,marcus2019neo,kraska2019sagedb} in the database community.
Recently, the database community recognized the potential of replacing traditional cardinality estimation methods by learning-based models (e.g., neural network, autoregressive model)~\cite{wang2020we,lan2021survey}.
Existing learning-based estimators can be classified into three categories: \emph{query-driven},
\emph{data-driven} and \emph{hybrid}.

\emph{Data-driven cardinality estimators}~\cite{hilprecht2019deepdb,yang2020neurocard} share the same idea with traditional cardinality estimation methods,
i.e., they hope to capture the correlations and distributions of data across the tables.
%Different from histogram-based and sampling-based methods, data-driven cardinality estimation approaches use complex learning models to learn the joint distribution of the tables~\cite{hilprecht2019deepdb,yang2020neurocard}.
%For example, 
$\deepdb$~\cite{hilprecht2019deepdb} adopts  relational sum product networks (RSPN) to capture the probability distribution among relations, and translates a query into the evaluations of probabilities and expectations based on RSPN.
$\naru$~\cite{yang2019deep} adopts autoregressive models, i.e., masked autoencoder~\cite{germain2015made} and transformer~\cite{vaswani2017attention}
to estimate the selectivity of equal and range predicates.
$\neuro$~\cite{yang2020neurocard} trains a single deep autoregressive model based on samples collected from the full outer join result of all relations.
The model can be used to answer complex queries with joins on any subset of the relations.

%$\mscn$~\cite{MSCN} and $\tlstm$~\cite{Guoliang} are two state-of-the-art deep learning solutions.
%Specifically, 
\emph{Query-driven cardinality estimators}~\cite{stillger2001leo,MSCN,Guoliang,hasan2020deep,dutt2019selectivity} formulate cardinality estimation as a regression problem.
The contents of queries and their true cardinalities are used as training data to learn a mapping from queries to cardinalities.
~\cite{dutt2020efficiently} uses regression techniques such as XGBoost, to train the model to produce approximate cardinality labels.
$\mscn$ transforms a query into a feature vector and uses a multi-set convolution network~\cite{zaheer2017deep} to map it to cardinality estimation. 
$\tlstm$ processes a query execution plan recursively following its tree structure using $\lstm$ (a kind of $\rnn$)~\cite{hochreiter1997long}.
%, which derives the embedding of a node from its feature vector and the embeddings of its two children.

%~\cite{wu2021unified, MSCN, Guoliang,dutt2019selectivity} extract useful information from both data and query samples.

\emph{Hybrid cardinality estimator}
$\uae$~\cite{wu2021unified} learns the joint data distribution among the tables as in the data-driven estimators, and uses query samples as auxiliary information at the same time.
With a unified deep autoregressive model, $\uae$ learns from data in an unsupervised manner and query samples in a supervised manner.

As we have discussed in Section~\ref{sec:intro}, existing cardinality estimators cannot achieve \emph{high accuracy} and \emph{fast inference} simultaneously, which are necessary for short end-to-end query execution time. Our $\lpce$ is general framework, which enjoys the fast inference of query-driven estimators and progressively refines estimations to correct large errors. We have shown that data-driven and hybrid estimators also have larger errors for complex queries, and thus may also benefit from our progressive cardinality estimation methodology.   

 

%In this work, we follow learning-based approaches in the \emph{query-driven} category as:
%(i) the study on cardinality estimation model is orthogonal to our $\lpce$ architecture for query re-optimization problem,
%as it can be used as the cardinality estimation model (i.e., $\lpcei$ model) in $\lpce$ directly;
%and (2) the estimation accuracy of \emph{data-driven} models rely on the quality of the data samples (used for model training). In some cases, accessing a large amount of original data may be infeasible due to privacy and security concerns. %Query-driven approaches have the benefit of treating sensitive data as a black box, which returns cardinalities for the given queries.   

%These errors are introduced by the interactions of multiple predicates and the correlations in the data~\cite{lohman2014query,wu2016sampling}, which makes it difficult for query optimizers to find the optimal execution plan.

\stitle{Query re-optimization} Although extensive efforts have been made to improve the accuracy of cardinality estimation, the errors can still be large for complex queries, e.g., those with multiple joins. 
Query re-optimization techniques~\cite{avnur2000eddies,kabra1998efficient,abdel2009rox,dutt2014plan,wu2016sampling, neumann2013taking} have been proposed to combat the influence of large estimation errors on query optimization.
The general idea is that the query optimizers first choose an initial execution plan, and then exploit extra knowledge to adjust to a better execution plan.
There are two classes of query re-optimization techniques.
(1) \emph{Re-optimizing during query execution.} For example, $\rox$~\cite{abdel2009rox} samples data from the intermediate results,
and tries different operator implementations and join orders on the samples to adjust the remaining execution plan.
(2) \emph{Re-optimizing before query execution.} For example, Wu et al.~\cite{wu2016sampling} use a sampling-based method to detect estimation errors and then adjust the execution plan before running it. Our $\lpce$ differs from these query re-optimization techniques in that they are sampling-based while $\lpce$ uses machine learning to exploit information in the executed sub-queries for estimation refinement.   


%Our $\lpce$ differs from~\cite{wu2016sampling} in two ways. First, $\lpce$ re-optimizes query execution plan during query runtime.
%Second, our $\lpce$ is learning-based while \cite{wu2016sampling} is sampling-based.
%
%In this work, we propose a novel learning-based solution (i.e., $\lpce$) to re-optimize query execution plan during execution.
%Different from the sampling-based technique in $\rox$, $\lpce$ exploits the information in the executed sub-queries using a machine learning model.


==> figures/8_concl.tex <==
\section{Conclusion}~\label{sec:concl}
We propose $\lpce$, a learning-based cardinality estimator that progressively refines the cardinality estimations during the query execution process. 
We observed that to reduce the end-to-end execution time of queries, both fast inference and high accuracy are necessary but no existing cardinality estimators can satisfy the two requirements simultaneously. 
Thus, $\lpce$ adopts a novel framework, which uses a query-driven estimator for fast initial estimation and exploits the executed sub-plans to correct large estimation errors for the remaining operators.
We propose techniques including node-wise loss function, knowledge distillation-based model compression and refinement model with three modules to instantiate $\lpce$.
Extensive experiments show that our $\lpce$ outperforms existing learning-based estimators in reducing the end-to-end execution time of queries, especially in worst cases.
There are many interesting problems in applying learning-based progressive cardinality estimation to speed up query execution, including devising tailored plan enumeration algorithms and improving the performance of data-driven or hybrid learning-based estimators, which we leave for future work.

%$\lpce$ consists of a \emph{cardinality estimation model} for initial estimation before query execution and a \emph{cardinality refinement model} that can progressively improve estimation accuracy in the query execution process. With techniques including node-wise loss function, knowledge distillation-based model compression and refinement model with three modules,
%$\lpce$ meets the requirements of high estimation accuracy, fast inference and progressive estimation refinement. 
